Uncovering Software-Based Power Side-Channel Attacks on Apple M1/M2 Systems

Traditionally, power side-channel analysis requires physical access to the target device, as well as specialized devices to measure the power consumption with enough precision. Recently research has shown that on x86 platforms, on-chip power meter capabilities exposed to a software interface might be used for power side-channel attacks without physical access. In this paper, we show that such software-based power side-channel attack is also applicable on Apple silicon (e.g., M1/M2 platforms), exploiting the System Management Controller (SMC) and its power-related keys, which provides access to the on-chip power meters through a software interface to user space software. We observed data-dependent power consumption reporting from such SMC keys and analyzed the correlations between the power consumption and the processed data. Our work also demonstrated how an unprivileged user mode application successfully recovers bytes from an AES encryption key from a cryptographic service supported by a kernel mode driver in MacOS. We have also studied the feasibility of performing frequency throttling side-channel attack on Apple silicon. Furthermore, we discuss the impact of software-based power side-channels in the industry, possible countermeasures, and the overall implications of software interfaces for modern on-chip power management systems.

==> bib <==
\begin{thebibliography}{1}

\bibitem{Nance:VMI}
K.~Nance, B.~Hay and M.~Bishop.
\newblock Virtual machine introspection: Observation or interference?
\newblock In {\em IEEE Symposium on Security and Privacy}, pages 32--37, Sep.
  2008.

\bibitem{Azmandian:vmmblid}
F.~Azmandian, M.~Moffie, M.~Alshawabkeh, J.~G. Dy, J.A.~Aslam, and D.R.~Kaeli.
\newblock Virtual machine monitor-based lightweight intrusion detection.
\newblock {\em ACM SIGOPS Operating Systems Review}, 45(2):38--53, July 2011.

\bibitem{zwang:hookp}
Z.~Wang, X.~Jian, W.~Cui and P.~Ning.
\newblock Countering kernel rootkits with lightweight hook protection.
\newblock In {\em Proceedings of the 16th ACM conference on Computer and
  communications security (CCS)}, pages 545--554, Nov. 2009.

\bibitem{pbd:xenacess}
B.D.~Payne, M.~Carbone and W.~Lee.
\newblock Secure and flexible monitoring of virtual machines.
\newblock In {\em Computer Security Applications Conference}, pages 385--397,
  Dec. 2007.

\bibitem{jiang:vmwatcher}
X.~Jiang, X.~Wang and D.~Xu. 
\newblock Stealthy malware detection through vmm-based ``out-of-the-box"
  semantic view reconstruction.
\newblock In {\em Proceedings of ACM conference on Computer and communications
  security (CCS)}, pages 128--138, Nov. 2007.

\bibitem{TG:livewire}
T.~Garfinkel and M.~Rosenblum.
\newblock A virtual machine introspection based architecture for intrusion
  detection.
\newblock In {\em Proceedings Network and Distributed Systems Security
  Symposium}, pages 191--206, 2003.

\bibitem{Dxu:dksm}
S.~Bahram, X.~Jiang, Z.~Wang J.~Rhee and D.~Xu.
\newblock DKSM: Subverting virtual machine introspection for fun and profit.
\newblock In {\em Proceedings of the 29th IEEE International Symposium on
  Reliable Distributed Systems (SRDS)}, Oct. 2010.

\bibitem{vmwall}
A.~Srivastava and J.T.~Giffin.
\newblock Tamper-resistant, application-aware blocking of malicious network connections.
\newblock In {\em International Symposium on Recent Advances in Intrusion Detection (RAID)}, pages 39--58, 2008.

\bibitem{Lares}
B.D.~Payne, M.~Carbone, M.~Sharif and W.~Lee.
\newblock Lares: An Architecture for Secure Active Monitoring Using Virtualization.
\newblock In {\em Proceedings of the IEEE Symposium on Security and Privacy }, May 2008.

\bibitem{nickle}
R.~Riley, X.~Jiang and D.~Xu.
\newblock Guest-Transparent Prevention of Kernel Rootkits with VMM-based Memory Shadowing.
\newblock In {\em  Proceedings of the 11th international symposium on Recent Advances in Intrusion Detection}, 2008.

\bibitem{cop}
N. L.~Petroni, T.~Fraser, J.~Molina and W. A.~Arbaugh.
\newblock Copilot-a coprocessor-based kernel runtime integrity monitor.
\newblock In {\em Proceedings of the 13th USENIX Security Symposium}, page 179--194, 2004.

\bibitem{hpc}
C.~Malone, M.~Zahran and R.~Karri.
\newblock Are Hardware Performance Counters a Cost Effective Way for Integrity Checking of Programs?
\newblock In {\em The Sixth ACM Workshop on Scalable Trusted Computing}, Oct. 2011.

\bibitem{vee}
J.~Du, N.~Sehrawat and W.~Zwaenepoel.
\newblock Performance profiling of virtual machines
\newblock In {\em Proceedings of the 7th ACM SIGPLAN/SIGOPS international conference on Virtual execution environments}, July 2011.

\bibitem{vtune}
Intel Inc.
\newblock Intel VTune Performance Analyzer.
\newblock http://software.intel.con/en-us/intel-vtune, 2010.

\bibitem{opro}
J.~Levon and P.~Elie.
\newblock Oprofile: A system profiler for linux.
\newblock http://oprofile.sourceforge.net, 2010.

\bibitem{perf}
\newblock Performance Counters for Linux.
\newblock http://lwn.net/Articles/310176, 2010.

\bibitem{kvm}
\newblock Kernel Based Virtual Machine.
\newblock http://www.linux-kvm.org/page/Main\_Page

\bibitem{qemu}
\newblock www.qemu.org/

\bibitem{dkom}
G.~Hoglund and J.~Butler
\newblock Rootkits: Subverting the windows kernel
\newblock Addison Wesley, Boston, USA, 2006




\end{thebibliography}


==> sections/threatmodel.tex <==
\begin{figure}
	\centerline{\includegraphics[width=2.5in]{figures/SPM_attack_example.png}}
	\caption{Ring-0 attacker compromises the confidentiality of a Trust Execution Environment using telemetry side-channel.}
	\label{fig:spm_attack_example}
	\vspace{-10pt}
\end{figure}
\subsection {Telemetry vs. Physical side-channel}\label{ss:necessary condition}
Fig. \ref{fig:spm_attack_example} depicts a typical telemetry side-channel attack. The victim program is executed in a Trusted Execution Environment (TEE) (e.g., ARM TrustZone\cite{Trustzone} and Intel SGX\cite{SGX}), in its own private region where even a privileged software attacker cannot directly read secret information from it. However, the secret information may be correlated with physical attributes (e.g., power, EM radiation, voltage, temperature, etc.) of the CPU(s) during workload execution. These attributes are further measured and aggregated by on-chip sensors or event counters and exposed to software as CPU-related telemetries. The adversary, if allowed to read the telemetries, may deduce secret information of the victim program. In this way, CPU telemetries become the proxy for an adversary to bypass isolation and retrieve secrets.

Compared with physical side-channel attacks, a telemetry side-channel attack requires neither physical access to the target system nor any additional measurement instrument. Moreover, it is usually difficult for a physical attack to isolate attributes of a specific component (e.g., CPU, memory, GPU) from that of the entire platform. In a telemetry side-channel attack, on-chip sensors may report finer-grained measurement for a specific component.
Conversely, a telemetry side-channel attack suffers from limited sampling frequency and resolution. First, an oscilloscope may have a sampling frequency fast enough to obtain cycle-accurate information of most modern CPUs, whereas a telemetry's sampling frequency is much slower, as it is bounded by on-chip monitor sampling frequency, telemetry aggregation frequency, and end-to-end delay when software polls the telemetry. Second, while resolution of physical side-channel data collection can be improved with better instruments, resolution of telemetry is bounded by on-chip sensor accuracy, which is usually relatively low and fixed. 

\iffalse
\begin{table}[t]
\caption{Comparison between Physical Probing and Telemetry}
\begin{tabular}{l|cc}\label{Table:pm-compared}
& \multicolumn{1}{c}{Physical Probing} & \multicolumn{1}{c}{Telemetry}   \\ \hline
Access method                                                     & {\color[HTML]{FE0000} Physical}           & {\color[HTML]{009901} Software}       \\ \hline
Extra instrument                                                  & {\color[HTML]{FE0000} Y}           & {\color[HTML]{009901} N}       \\ \hline
Measurement domain                                                    & {\color[HTML]{FE0000} Coarse-grained}           & {\color[HTML]{009901} Fine-grained}       \\ \hline
Resolution                                                          & {\color[HTML]{009901} High}        & {\color[HTML]{FE0000} Limited} \\ \hline
\begin{tabular}[c]{@{}l@{}}Sampling frequency\end{tabular} & {\color[HTML]{009901} High}        & {\color[HTML]{FE0000} Limited}
\end{tabular}
\end{table}
\fi

\subsection {Threat model}\label{ss:threat model}
In this paper, we consider the threat that a software adversary utilizes information collected from telemetries to perform side-channel attacks to retrieve secrets from a victim. By default, only privileged adversary is permitted to access telemetry interfaces. But the attack surface may expand if a telemetry interface is exposed to less-privileged users. Depending on the adversary, the victim can be ring 0/3 software, a TEE, or hardware/firmware.
We enumerate possible threats as below, based on the privileges of attackers and victims:
\begin{enumerate}[leftmargin=0.35cm]
\itemsep0em 
    \item Ring-0/3 $\xrightarrow{attack}$ TEE: A TEE is an isolated environment that has neither ring-3 nor ring-0 software in its TCB. A malicious ring-0/3 adversary may exploit telemetries to deduce secrets from a TEE. Moreover, in a cloud environment, a malicious cloud service provider (CSP) may also exploit telemetries to attack TEE executed by a client.
    \item Ring-3 $\xrightarrow{attack}$ Ring-0/3: If a telemetry is accessible by ring-3 software, a malicious userland application may use it to steal confidential information of another ring-3 application or a program running in the kernel space.
    \item Ring-0/3 $\xrightarrow{attack}$ Hardware/Firmware assets: On modern computing platforms, there are secrets stored in hardware and firmware that should not be exposed to OS or users. Examples of such secrets include hardware keys for crypto engines or manufacturer's confident data protected by system management mode (SMM). telemetries open a potential avenue for malicious user applications and OS to extract the secrets. 
\end{enumerate}
